Generalizing in the Real World with Representation Learning

Machine learning (ML) formalizes the problem of getting computers to learn from experience as optimization of performance according to some metric(s) on a set of data examples. This is in contrast to requiring behaviour specified in advance (e.g. by hard-coded rules). Formalization of this problem has enabled great progress in many applications with large real-world impact, including translation, speech recognition, self-driving cars, and drug discovery. But practical instantiations of this formalism make many assumptions - for example, that data are i.i.d.: independent and identically distributed - whose soundness is seldom investigated. And in making great progress in such a short time, the field has developed many norms and ad-hoc standards, focused on a relatively small range of problem settings. As applications of ML, particularly in artificial intelligence (AI) systems, become more pervasive in the real world, we need to critically examine these assumptions, norms, and problem settings, as well as the methods that have become de-facto standards. There is much we still do not understand about how and why deep networks trained with stochastic gradient descent are able to generalize as well as they do, why they fail when they do, and how they will perform on out-of-distribution data. In this thesis I cover some of my work towards better understanding deep net generalization, identify several ways assumptions and problem settings fail to generalize to the real world, and propose ways to address those failures in practice.

==> 2-Remerciements.tex <==
% Remerciements / Acknowledgements
%
%  Grâce aux remerciements, l'auteur attire l'attention du lecteur
% sur l'aide que certaines personnes lui ont apportée, sur leurs
% conseils ou sur toute autre forme de contribution lors de la
% réalisation de son mémoire. Le cas échéant, c'est dans cette section
% que le candidat doit témoigner sa reconnaissance à son directeur de
% recherche, aux organismes dispensateurs de subventions ou aux
% entreprises qui lui ont accordé des bourses ou des fonds de
% recherche.
\ifthenelse{\equal{\Langue}{english}}{
	\chapter*{ACKNOWLEDGEMENTS}\thispagestyle{headings}
	\addcontentsline{toc}{compteur}{ACKNOWLEDGEMENTS}
}{
	\chapter*{REMERCIEMENTS}\thispagestyle{headings}
	\addcontentsline{toc}{compteur}{REMERCIEMENTS}
}
%
I am first and for|most grateful to my family for their invaluable love and support - including all my extended family and family by choice. From a young age you've made me feel the world is full of kind, interesting, intelligent, creative people who will be there for each other and for me. I'm lucky to have you all. I'm especially grateful to my parents, Laurie and Ken, to Keir, Aaricia, Amiani, Lisa, Mauri, Maya, and Mason for making me feel at home wherever I am, and to David, Don, Val, Susan, Clint, and Gretchen for welcoming me into your families. 

This theis 


==> 9-Annexes.tex <==
%%
%%  Annexes
%%
%%  Note: Ne pas modifier la ligne ci-dessous. / Do not modify the following line.


\ifthenelse{\equal{\Langue}{english}}{
	\addcontentsline{toc}{compteur}{APPENDICES}
}{
	\addcontentsline{toc}{compteur}{ANNEXES}
}

% Résumé du mémoire.
%
\chapter*{SUMMARY}\label{sec:summary}
%\addcontentsline{toc}{compteur}{SUMMARY}




    I introduce my work with a review of artificial intelligence (AI), machine learning (ML), and deep learning concepts and terminology, including a review of recent literature in understanding generalization with deep networks. 
    %Each following chapter also presents a context-specific background and literature review. 
    
The next chapter summarizes two works exploring memorization and generalization behaviour of deep networks [1,2], which discuss a series of experiments contrasting learning behaviour on noise vs. real data distributions. These works provide strong empirical evidence for important elements of folk wisdom about deep nets, including the dependence of deep network learning behaviour on the distribution of training data, and that simple patterns which generalize well are learned first, before memorization/overfitting.  The findings from these highly-cited works have been supported in a wave of empirical and theoretical follow-up studies.
    
After that, I cover work from [3] on a regularization method called Zoneout. Dropout, which randomly sets some activations of a deep network to 0, is a very widely used regularization technique for feed-forward neural networks, enabling them generalize well on a much wider range of atemporal real-world data (e.g.images). But in recurrent neural networks (RNNs), widely used for temporal data, where activations from one timestep become inputs for the next timestep, dropout causes instability and vanishing gradients. Our work proposes a simple alternative, to randomly set activations to their previous value, enabling RNNs to get all the regularization benefits of dropout. Zoneout was widely adopted in real-world applications of RNNs.
    
Next, I present an empirical exploration of learned representations for video data. In this work we propose and investigate a simple predictive task, fill-in-the-blank, and introduce a large dataset for this task. We demonstrate through extensive experiments, including human evaluations, that this simple task significantly improves video description quality, as well as 2D and 3D representations of video data. The usefulness of this simple task has been confirmed in many other works, notably in language modelling, where it is called masking. Large masked language models currently form the basis of Google search results.
    
The next chapter summarizes two works examining real-world consequences of distributional shift, and proposes two methods for responsible AI development that could help prevent or address these consequences: unit tests and sandboxes. First I summarize [5], where we define auto-induced distributional shift (ADS) as shift caused by the presence or actions of an algorithm/agent. We look at conditions under which an incentive for ADS could be revealed by a learning setup, and demonstrate the potential real-world consequences of incentives for ADS in content recommendation systems. 
    While ADS is not categorically undesirable, in some settings like content recommendation, it may be an unacceptable means of solving the problem, but our performance metrics fail to specify this. For example, an algorithm might be able to do well according to predictive accuracy by changing user interests to make them easier to predict, or driving away hard-to-predict users. We develop simple unit tests for reinforcement learning and online supervised learning systems, which detect whether a system may be vulnerable to incentives to achieve performance via ADS. Unit tests like this could form an important component of testing or auditing real-world AI systems. 
    
    Next, I summarize work in developing a detailed agent-based epidemiological simulator, tuned to real virological and behavioural data for Covid-19. This simulator serves as a sandbox for comparing and testing novel digital contact tracing (DCT) methods and other public health interventions. This approach allowed us to discover and deal with two important issues for DCT methods: (1) generating sufficient training data to be robust to a variety of real-world conditions, and (2) a successful DCT method will cause a shift in data, by preventing cases of the disease, and training needs to account for this. Sandboxing with an agent-based simulator is a general approach for evaluating representation learning systems prior to real-word deployment. In the context of digital health, among other benefits this approach could contribute to more efficient design of randomized control trials.
    
   Finally, I cover [5], which develops and tests a novel approach to digital contact tracing (DCT) for Covid-19. This approach casts the problem of DCT as distributed inference of individual-level risk of Covid-19, measured as individual infectiousness. In order to estimate this quantity privately on individual smartphones, we leverage the simulator from [6] to provide rich training data, including variables such as viral load which are not feasibly available at scale in real data, and train set-based predictors offline. We show that this approach provides an excellent trade-off in managing disease: reducing cases more than any tested method, while requiring very little quarantine of healthy individuals. This latter point is important for preventing and addressing pandemic fatigue, which has been shown to erode trust and compliance with public health measures.
   
   I conclude with some observations and takeaways from these works for effective real-world generalization, and identify next steps for research improving generalization of AI systems in realistic settings.

\newpage 
\textbf{In summary}, this thesis contains content verbatim from [2][3][4][7] in Chapters 2, 3, 4, 6 respectively, and selected content adapted from [1] and [5,6] for Chapters 2 and 5 respectively. Each chapter is self-contained, with background and appendices presented within the chapter when relevant.
%To preserve flow, works with substantial content not focused on in this thesis, [1][5][6], are presented in appendices. 

\begin{itemize}\footnotesize
    \item[{[1]}] Devansh Arpit†, Stanislaw Jastrzebski†, Nicolas Ballas†, David Krueger†, Emmanuel Bengio, Maxinder S Kanwal, Tegan Maharaj, Asja Fischer, Aaron Courville, Yoshua Bengio, Simon Lacoste-Julien. 2017. A closer look at memorization in deep networks. International Conference on Machine Learning (ICML).

    \item[{[2]}] Tegan Maharaj, David Krueger, and Tim Coojimans.  2017.  Memorization in recurrent neural networks. International Conference on Machine Learning (ICML) workshop on Principled Approaches to Deep Learning (PADL).

    \item[{[3]}] David Krueger†, Tegan Maharaj†, János Krámar, Mohammad Pezeshki, Nicolas Ballas, Nan Rosemary Ke, Anirudh Goyal, Yoshua Bengio, Aaron Courville, Christopher Pal. 2017. Zoneout: Regularizing RNNs by randomly preserving hidden activations. International Conference on Learning Representations (ICLR).

    \item[{[4]}] Tegan Maharaj, Nicolas Ballas, Anna Rohrbach, Aaron Courville, Christopher Pal. 2017. A dataset and exploration of models for understanding video data through fill-in-the-blank question-answering. IEEE Conference on Computer Vision and Pattern Recognition (CVPR).

    \item[{[5]}] David Krueger, Tegan Maharaj, Jan Leike. 2019. Revealing the Incentive to Cause Distributional Shift. International Conference on Learning Representations (ICLR) SafeML workshop.

    \item[{[6]}] Prateek Gupta†, Tegan Maharaj†, Martin Weiss†, Nasim Rahaman†, Hannah Alsdurf††, Nanor Minoyan††, Soren Harnois-Leblanc††, Joanna Merckx††, Andrew Williams††, Victor Schmidt, Pierre-Luc St-Charles, Akshay Patel, Yang Zhang, David L. Buckeridge, Christopher Pal, Bernhard Scholkopf, Yoshua Bengio. 2021. Proactive Contact Tracing. Public Library of Science (PLoS) Medecine  (in submission).

    \item[{[7]}] Yoshua Bengio†, Prateek Gupta†, Tegan Maharaj†, Nasim Rahaman†, Martin Weiss†, Tristan Deleu, Eilif Muller, Meng Qu, Victor Schmidt, Pierre-Luc St-Charles, et al. 2020. Predicting infectiousness for proactive contact tracing. International Conference on Learning Representations (ICLR).

\end{itemize}
\vspace{-2mm}
\hspace{5MM} † indicates equal contribution
\vspace{3mm}

\textbf{A note on publication venues}: Conferences, including NeurIPS, ICML, ICLR, and CVPR, are among the top scholarly venues for research in the field of machine learning, comparable to journals in many other academic fields. They publish full-length papers with full peer-review. Workshops are a component of conferences which present short papers (around 4 pages), typically early results, to a more specialized audience than the overall conference. They are peer-reviewed, but non-archival.


\chapter*{PREAMBLE}
%\addcontentsline{toc}{compteur}{PREAMBLE}
\pagestyle{pagenumber}
%

\section*{A. Original contributions \& relation to theme}
%\addcontentsline{toc}{section}{A. Original contributions \& relation to theme}

The theme of my thesis is real-world generalization with representation learning. My work in this thesis makes the following original contributions in this theme:

\vspace{2mm}
\textit{Note: I emphasize here individual contributions I made in collaborative works, but these of course depend on, and cannot be cleanly separated from, the contributions of other authors and of the works as a whole, for which credit is due to all the authors as a team. More detailed information on my contributions to each work is provided at the beginning of each section in the thesis.}

\begin{enumerate}[itemsep=2pt]
    \item \textbf{Review} of recent progress understanding the factors influencing real-world generalization of deep networks, contextualizing the works presented in this thesis and providing a foundation for future work in this fast-growing area. (CH. \ref{sec:introduction})
   
    \item \textbf{Empirical exploration} of memorization and generalization with recurrent neural networks, generating insight on similarities and differences from feed-forward networks (and thereby the effects of depth on memorization). Theory works tend to focus on atemporal data, but many data of real-world interest (e.g. many data relating to climate, social science, and health) have important temporal variation. The `empirical theory' approach of this paper is generally useful for generating the kinds of insights and intuition that are helpful for designing systems that generalize in the real world. Understanding when neural networks will memorize (vs. learn underlying patterns of) training examples also helps us better design new methods and training regimes.  (CH. \ref{sec:memgen})
    
    \item Development and empirical evaluation of a novel regularization method for recurrent neural networks, \textbf{Zoneout}, with insight into the role of regularization for gradient propagation. Dropout became so quickly and widely adopted because of how well it encourages generalization, even in relatively low data regimes, common with real-world data. Zoneout allows the same benefits for temporal data. (CH. \ref{sec:zoneout})
    
    \item Proposal and comprehensive evaluation of a \textbf{fill-in-the-blank} dataset for benchmarking video models, with baseline results and challenge evaluation platform. Demonstration that the simple predictive task of filling-in-the-blank on captions (similar to and preceding masked language modelling) improves representations of video data and is better aligned to human evaluations than commonly-used word-overlap measures such as BLEU. Designing better-aligned tasks and methods of evaluation are important for ensuring real-world generalization. (CH. \ref{sec:moviefib})
    
    \item Co-definition of the term \textbf{auto-induced distributional shift (ADS)}, and exposition of the role it can play in content recommendation. The assumption that data are sampled iid (independently and identically distributed) is often made in machine learning theory, but it rarely holds for real-world data. However, the practical consequences of this assumption failing to hold are seldom investigated. We show the impact this can have in content recommendation, which is increasingly prevalent in peoples' daily life via search, social media, etc. Investigating the practical consequences of assumptions is an important aspect of ensuring good generalization in the real world.
    %In general, we highlight the fact that typical training regimes specify only the \textit{ends} we want an algorithm to reach, and not the \textit{means} we want them to use -  
    (CH. \ref{sec:dist})
    
    \item Proposal of the approach of \textbf{unit-testing} for recognizing behaviours that are difficult to specify in advance of training, but easy to recognize in a trained model. Contribution to developing unit-tests for models that might undesirably or unexpectedly achieve performance via ADS. Our unit test provides a practical way to assess when algorithms might follow an incentive to achieve performance via ADS - i.e., when they might generalize in an undesirable way in the real world. (CH. \ref{sec:dist})
    
    \item Proposal of the approach of \textbf{sandboxing} for training, evaluating, and comparing algorithms prior to real-world deployment by using Agent-Based Models (ABM) simulators; instantiation and testing of this approach in the development of a detailed ABM for simulation of Covid-19 epidemiology (COVI-AgentSim). The Covid-19 pandemic has had a huge impact on daily life for most people. New technologies like digital contact tracing could help lessen this impact and protect people in this and future pandemics. But like any intervention relating to health and welfare, it is essential that they be thoroughly tested. In general the approach of sandboxing with an ABM is helpful for evaluating the generalization capabilities (among other aspects) of a model prior to deployment in the real world, and specifically COVI-AgentSim helps us develop better DCT methods for Covid-19. (CH. \ref{sec:dist})
    
    \item Co-development of the method of \textbf{predictive contact tracing}, including formalizing the problem as distributed inference of infectiousness, and use of COVI-AgentSim as an evaluation sandbox, allowing us to compare models as well as to recognize and address issues of ADS in contact tracing.  This provides a good example of the kinds of important phenomena we can discover and address via sandboxing - we often do not know in advance how to speficy which kinds of generalization are desirable, but sandboxing can help us target desirable properties in practice. Distributed inference performed as we did is also generally useful for large-scale privacy-preserving use of representation learning for individual-level risk estimation, which could be important for many real-world tasks such as quantifying negative externalities from pollution, climate change, etc. (CH. \ref{sec:covi})
\end{enumerate}





\section*{B. Notes on scope (what this thesis is not)} \label{sec:Limitations}
%\addcontentsline{toc}{section}{B. Notes on scope (what this thesis is not)}
%This gives background for the things I address in this thesos: regulariazing to improve generaliazaion, why exactly this helps (memgen), when specificatoins fail to accurately capture what we 'actually wanted', and some practical ways to deal with that.

There are many aspects of generalizing in the real world that are not addressed by this thesis. I focus on the techniques that have dominated real-world AI applications in recent years, and the dominant paradigms of theory for understanding A: i.e. deep neural networks used in mostly-supervised settings, described in the language of probability and statistical machine learning. This thesis does not cover, for example, tree-based methods, bayesian ML, causal ML, information theory, complex systems theory, evolutionary methods, or reinforcement learning. Nor does it cover much of the extensive data science work required to build datasets suitable for large-scale learning (although this is touched on in Chapter 4).

Perhaps most notably though, I focus here on the technical side of addressing what are fundamentally socio-technical systems.  A solely technical approach to real-world generalization (and by extension, responsible AI development) is doomed to failure. Artificial intelligence systems are human systems, built by humans and used by, on, and for humans. 
%However, I Engages with the dominant paradigms of ML/A, in order to make concrete progress, but responsible AI development requires a broader lense than presented here. 
Experience and information about the world are not limited to or necessarily easily cast as sets of data examples; untidy data and other ways of knowing about the world are sorely under-represented in ML, AI, deep learning, and data science. 

However, in order to make concrete progress, I believe it's necessary and useful to engage with the dominant paradigms of the field, and this thesis reports my work in doing that. While the last chapters touch on some aspects of systems modeling, alignment, and human-computer interaction, these are hugely important areas I believe will see an explosion of interest in years to come. I hope that this thesis comes to fit in a larger context of multi-disciplinary, multi-stakeholder efforts towards more informed, responsible, and beneficial use of AI.
%This dissertation covers several of my works exploring generalization behaviour of deep networks


\section*{C. Notes on notation}
%\addcontentsline{toc}{section}{C. Notes on notation}

 Because deep networks very typically operate on vectors of data, and not scalar-valued data, for consistency I use vector notation throughout, without loss of generality to the scalar case as scalars can be considered as 1-D vectors. Boldface italics are used to indicate a vector-valued function, e.g. \textbf{\textit{f}}. Capital letters in boldface are used for matrices, e.g. \textbf{W}, lower-case letters in boldface for vectors, e.g. \textbf{x}, boldface with an index for a particular element of the vector, e.g. $\textbf{x}_1$, and italic non-boldface to indicate any-and-every element of the vector, e.g. $\textit{y}$. This vector notation is prioritized over the conventions of probability, where random variables are typically denoted with capital (non-boldface) characters and values of random variables indicated with lower-case (non-boldface) type.  A boldface \textbf{1} or other number is used to indicate a vector where each element is that number. To avoid excessive boldface, function names with more than one letter are not bolded, even if they return a vector. For example, $\textit{exp}^\textbf{x}$ indicates a vector where each element is the number $e$ to the power of the corresponding element of \textbf{x}. 





\section*{D. Outline of content in this thesis}
%\addcontentsline{toc}{section}{D. Outline of content in this thesis}

\textit{For a full summary, see SUMMARY in the previous section. }

The introduction first presents a background to AI and ML, with a focus on generalization, including a review of recent works. Each chapter then first gives the full citation for article(s) covered in that chapter, and some contextual notes, before reproducing or summarizing the article(s). Each chapter is self-contained, with introduction and literature review and any appendices included as they were published. 

I begin with work empirically examining generalization behaviour of deep networks in \textbf{Chapter 2}, where we observe that generalization and learning behaviour depend on the data distribution, and regularization contributes significantly to generalization at the expense of memorization \cite{arpit2017,memRNN}.  %implication: we can't just offload/abdicate responsibility by saying ``it's all data bias'' .Also, presence of reg alone reduces mem, whatever the reg. (incentive/pressure away from blind opt)

\textbf{Chapter 3} then integrates my co-first author work on an explicit regularizer for recurrent neural networks which confers the benefits of dropout while improving gradient flow to early timesteps \cite{zoneout}. 
%implication temporal data had yet to see the same boom in applications as ff, particularly for small-data regimes where reg is important.

\textbf{Chapter 4} integrates my first-author work examining evaluation of video models, and proposing the simple predictive task of `fill-in-the-blank' (in language modelling, now known as masking) as a means of improving learned representations \cite{moviefib}.
%implication: again, not trivial to get same perf for spatiotemporal models as ff. eval metric makes a difference not just on sample complexity but also what rep we end up with / predictive tasks give implicit regularization toward good rep (cf first works; generalizes better)

\textbf{Chapter 5} covers 2 works addressing auto-induced distributional shift (ADS) (i.e. shift caused by AI systems) in content recommendation \cite{hiads} and Covid-19 epidemiology \cite{gupta2020covisim} respectively. These works also serve to introduce two practical techniques for ensuring better real-world generalization: unit-testing and sandboxing. 
%In the former, we propose a unit-testing approach for detecting which systems might follow incentives to cause distributional shift as a means of achieving good performance. In the latter, we address issues with ADS in practice via iterative retraining (on successive shifts), a strategy we were able to develop by using an Agent-Based Model (ABM) of Covid-19 as a 'sandbox' \cite{gupta2020covisim}.

Finally, \textbf{Chapter 6} integrates the co-first author paper \cite{gupta2020covisim}  in which we cast the problem of digital contact tracing (DCT) as distributed inference of infectiousness, and leverage our ABM sandbox to train predictors offline. We show that this strategy, leveraging the weak signals available on smartphones, enables proactive recommendations that effectively prevent spread of disease while requiring very little quarantine of healthy individuals.

I conclude by identifying some key takeaways and approaches from my work for real-world generalization, and discuss next steps.




==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Copyright (c) 2005 Matti Airas <Matti.Airas@hut.fi>

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions:

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software.

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE.

TEXINPUTS += :./dia:./gnuplot:./images:./modules
export TEXINPUTS

SRC	= Document.tex
LATEX	= latex -output-format=dvi
PDFLATEX= pdflatex
BIBTEX	= bibtex
XDVI	= xdvi -paper us
DVIPDF  = dvipdfm -p letter

COPY     = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi
RERUN    = "(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"


$(SRC:%.tex=%.pdf): $(SRC) $(SRC:%.tex=%.bib) images $(shell ls -1 images/*.eps 2> /dev/null)
	$(COPY); $(PDFLATEX) $(SRC)
	@egrep -c $(RERUNBIB) $(SRC:%.tex=%.log) && ($(BIBTEX) $(SRC:%.tex=%); $(COPY); $(PDFLATEX) $(SRC)); true
	@egrep -q $(RERUN) $(SRC:%.tex=%.log) && ($(COPY);$(PDFLATEX) $(SRC)); true
	@egrep -q $(RERUN) $(SRC:%.tex=%.log) && ($(COPY);$(PDFLATEX) $(SRC)); true
	@if cmp -s $(SRC:%.tex=%.toc) $(SRC:%.tex=%.toc.bak); then true; else $(PDFLATEX) $(SRC); fi
	@rm -f $(SRC:%.tex=%.toc.bak)
	@egrep -i "(Reference|Citation).*undefined" $(SRC:%.tex=%.log); true

$(SRC:%.tex=%.dvi): $(SRC) $(SRC:%.tex=%.bib) images $(shell ls -1 images/*.eps 2> /dev/null)
	$(COPY); $(LATEX) $(SRC)
	@egrep -c $(RERUNBIB) $(SRC:%.tex=%.log) && ($(BIBTEX) $(SRC:%.tex=%); $(COPY); $(LATEX) $(SRC)); true
	@egrep -q $(RERUN) $(SRC:%.tex=%.log) && ($(COPY);$(LATEX) $(SRC)); true
	@egrep -q $(RERUN) $(SRC:%.tex=%.log) && ($(COPY);$(LATEX) $(SRC)); true
	@if cmp -s $(SRC:%.tex=%.toc) $(SRC:%.tex=%.toc.bak); then true; else $(LATEX) $(SRC); fi
	@rm -f $(SRC:%.tex=%.toc.bak)
	@egrep -i "(Reference|Citation).*undefined" $(SRC:%.tex=%.log); true

images:
	@if [ -d dia ]; then cd dia; ${MAKE} -s -j 2; fi
	@if [ -d gnuplot ]; then cd gnuplot; ${MAKE} -s -j 2; fi

show: $(SRC:%.tex=%.dvi)
	@$(XDVI) $< &

%.pdf:	%.dvi
	@$(DVIPDF) -z9 -o $@ $<

pdf: $(SRC:%.tex=%.pdf)

clean:
	@rm -f *.aux *~ $(SRC:%tex=%){dvi,pdf,bbl,blg,log,out,lof,lot,loa,toc,app}

all_clean: clean
	@if [ -d dia ]; then cd dia; ${MAKE} clean; fi
	@if [ -d gnuplot ]; then cd gnuplot; ${MAKE} clean; fi

archive: all_clean
	@tar cjf Backup`date '+%Y%m%d'`.tar.bz2 images/* dia/* gnuplot/* *.{tex,sty,bst} Makefile

final:
	@head -n 1 $(SRC) | grep -q draft && (echo '1s/draft/final/'; echo 'w') | red $(SRC) > /dev/null 2>&1; true
	${MAKE}

draft:
	@head -n 1 $(SRC) | grep -q final && (echo '1s/final/draft/'; echo 'w') | red $(SRC) > /dev/null 2>&1; true
	@${MAKE}

help:
	@echo "Template LaTeX pour mémoires et thèses"
	@echo
	@echo "Utilisation:    make [options]"
	@echo
	@echo "  make            (Re)compilation du fichier LaTeX"
	@echo "  make pdf        Génération d'un fichier PDF"
	@echo "  make final      (Re)compilation du fichier LaTeX en mode Final"
	@echo "  make draft      (Re)compilation du fichier LaTeX en mode Draft"
	@echo "  make show       (Re)compilation et démarrage de XDVI"
	@echo "  make clean      Effacement des fichiers générés par LaTeX"
	@echo "  make all_clean  Effacement des fichiers générés par LaTeX et autres répertoires"
	@echo "  make archive    Génération d'un fichier archive avec la date du jour"
	@echo "  make images     Génération de toutes les images"
	@echo

.PHONY	: show clean all_clean pdf archive final draft help images


==> RM6-Revue_litterature.tex <==
\Chapter{REVUE DE LITTÉRATURE / LITERATURE REVIEW}\label{sec:RevLitt}

TODO

